Magnetic Distortion Resistant Orientation Estimation

Inertial Measurement Unit (IMU) sensors, including accelerometers, gyroscopes, and magnetometers, are used to estimate the orientation of mobile devices. However, indoor magnetic fields are often distorted, causing the magnetometer's readings to deviate from true north and resulting in inaccurate orientation estimates. Existing solutions either ignore magnetic distortion or avoid using the magnetometer when distortion is detected. In this paper, we develop MDR, a Magnetic Distortion Resistant orientation estimation system that fundamentally models and corrects magnetic distortion. MDR builds a database to record magnetic directions at different locations and uses it to correct orientation estimates affected by magnetic distortion. To avoid the overhead of database preparation, MDR adopts practical designs to automatically update the database in parallel with orientation estimation. Experiments on 27+ hours of arm motion data show that MDR outperforms the state-of-the-art method by 35.34%.

==> Bottleneck.tex <==
\vspace{-1mm}
\section{Observation on Magnetic Distortion}
\vspace{-1mm}
\label{secMotivation}
% Existing orientation estimation methods assume the magnetometer reading is the magnetic north in GRF, which causes an error in magnetic calibration.
Existing orientation estimation methods assume that the magnetic field directions in GRF are constant, while magnetic distortion makes the directions largely vary, causing significant error in magnetic calibration.
We conduct experiments to investigate the impact of magnetic distortion on orientation estimation (Section \ref{muse in distortion}). 
Then, we study the temporal and spatial properties of magnetic distortion (Section \ref{DBdesign}), which motivates us to model magnetic distortion with a database. 


To visualize distortion, we scan the magnetic field in a corridor.
Figure \ref{figScan} shows the angular difference between the magnetic direction measured at every location and the average magnetic direction of all locations.
Darker block means larger difference.
% From the measurement results, we see that the distribution of the magnetic field varies dynamically in a small area.
% We can see that magnetic field directions at different locations largely deviate from the average direction.
% Magnetic fingerprint methods for localization \cite{shu2015magicol, wang2021mvp, xie2014maloc, ho2020using, shao2016location, DEVRIES2009535, geomag, ahrs} are developed based on the very existence of distortion.
% and further stress this impact.
% Our experiments also show that magnetic field distortion exists at various kinds of daily-visit places.
% Details can be found in Section \ref{data}.
% MUSE and some other solutions, which always trust magnetometer reading as an unchanging global direction, suffer from magnetic distortion.
% MUSE and some other solutions, which always trust magnetometer reading as an constant global direction, suffer from magnetic distortion.
To quantify distortion magnitude, we define it as the deviation of magnetic field directions in a local area (e.g., the whole corridor), i.e., the average angular difference between the magnetic field directions at all locations and the average magnetic field direction of all locations.
% Using the corridor shown in Figure \ref{figScan} as example, the magnetic distortion will be the average of 



% \vspace{-1mm}
% (the same magnitude shown in Figure \ref{figScan}).
% We use the deviation of magnetic field directions, distortion, to describe the level of magnetic distortion in an area.
% \begin{equation}
%     dev_M = \overline{\angle(\overrightarrow{M} \cdot \overline{\overrightarrow{M}})}
% \end{equation}

\vspace{-1mm}
\subsection{Impact of Magnetic Distortion on Orientation Estimation} \label{muse in distortion}
\vspace{-0.5mm}
% To demonstrate the impact of magnetic distortion on orientation estimation, we use MUSE as an example, and test its performance under different distortion levels.
MUSE and other solutions, which always trust magnetometer reading as an constant global direction, suffer from magnetic distortion.
To quantify this impact, we test MUSE under different simulated distortion levels.
% To cancel the influence of other factors like motion pattern and motion speed, we generate data traces based on real arm motion data of one hour, and only control the magnetometer to simulate different distortion levels.
To simulate different distortion levels, we generate data traces based on real arm motion data of one hour, and only modify the magnetometer to simulate different distortion levels.
For the method to generate data with simulated distortion, please refer to Appendix \ref{appendix}.
% which is the difference of the magnetic direction measured at every location and the average magnetic direction of all locations.
% To cancel the influence of other factors like motion pattern and motion speed, we generate data traces based on a large amount of data traces we measured for evaluation in Section \ref{data}.
% In this dataset, we know the ground truth of the watch's orientation and location by a ground truth data collection system developed in \cite{miao}.
% We first transform the average magnetic field direction (usually north) from GRF into WRF, using the reverse of the ground truth orientation $\Theta_0^{-1}$:
% % (acquired in Section \ref{ground truth}): 
% $\overrightarrow{N}_{WRF}=\overrightarrow{N}_{GRF}\cdot\Theta_0^{-1}$ 
% \highlight{
% (the ground truth orientation is acquired via an accurate data collection system (to be introduced in Section \ref{ground truth})).
% }
% Based on this magnetic field direction in WRF, and the original magnetometer measurement direction $\overrightarrow{M}$ (measurement in WRF), we calculate a linear combination: $k_c\cdot\overrightarrow{M} + (1-k_c) \overrightarrow{N}_{WRF}$, with a ratio $k_c$.
% We normalize and use this new direction as the simulated magnetometer input.
% Via tuning $k_c$, we generate data with different distortion magnitude.
Figure \ref{muse_devM} shows the orientation error of MUSE.
As distortion rises from 6.72° to 44.89°, orientation error increases from 21.95° to 48.07°, showing a large impact by magnetic distortion.
% However, magnetic distortion can rise to 50° in real life, according to data we collected.



% While in Figure \ref{muse_devM}, as $err_G$ increases from 6° to 20°, CF performance changes little.
% The different range of X-axis of distortion and $err_G$ is because distortion does have larger range than $err_G$, corresponding to the distribution shown in Figure \ref{GM2}.
% Meanwhile $err_G$ has little effect on Gyro+Mag, due Gyro+Mag does not use magnetometer, except for the initialization process. Same for distortion to Gyro+Acc. 
% Gyro+Acc is even more sensitive to the variation of $err_G$, because accelerometer is the calibration for it. Same distortion to Gyro+mag.

% \textbf{Limitations of Existing Solutions:}
% Earth magnetic field usually has an magnitude around $45\mu T \sim 60\mu T$, and a certain angle with the gravity direction, mainly depending on the latitude.
% % Prior works \cite{fan2017adaptive} and \cite{ahrs} propose to use the magnetic field magnitude and the angle between magnetic field direction and gravity direction to detect magnetic distortion.
% Prior works \cite{fan2017adaptive, ahrs} propose to observe the abnormality in these two factors to detect magnetic distortion, while \cite{madgwick} only uses the magnitude.
% They use magnetometer less as distortion rises, in order to avoid the negative impact of magnetic distortion.
% % These methods are aware of magnetic distortion and try to avoid it.
% However, they also miss the opportunity of magnetic calibration, thus when distortion is high, they suffer from either magnetic distortion or the absence of magnetic calibration.
% Instead, we propose a novel system that models and corrects magnetic distortion in orientation estimation, even when distortion is high.
% \vspace{-1mm}
% In this paper, we perform magnetic calibration using distorted magnetic field within a novel system design. 
% We will borrow the idea from 
% \aliasSystem.

% As a result, the magnetic calibration process will calibrate orientation with a wrong anchor, and increase the estimation error.

% Now that traditional CF never updates its anticipation of $\overrightarrow{anchor_M}$, while the true $\overrightarrow{anchor_M}$ is changing, $\overrightarrow{anchor_M}$ will guide magnetometer to perform calibration in a wrong direction.
% % Unlike accelerometer having linear acceleration affecting its measurement on gravity, magnetometer is pure.
% Thus we conclude that the error in magnetometer calibration comes from \textbf{'calibrating true $\overrightarrow{e_{mag}}$ with a false $\overrightarrow{anchor_M}$'}.



\begin{figure*}[ht]
    \vspace{-1mm}
    \hfill
    \begin{minipage}[t]{0.26\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/sensys_muse_devM.pdf}
         \vspace{-7mm}
        % \caption{Impact of different magnetic distortion levels.}
        \caption{Impact of magnetic distortion on orientation error.}
        % \vspace{0cm}
        \label{muse_devM}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.25\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/mobi_chrono.pdf}
         \vspace{-7mm}
        \caption{Temporal stability of the magnetic field.}
        % \vspace{0cm}
        \label{temporal}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/sensys_spatial.pdf}
         \vspace{-7mm}
        \caption{Spatial correlation of the magnetic field.}
        % \vspace{0cm}
        \label{spatial}
    \end{minipage}
    \hfill
    \vspace{-4mm}
\end{figure*}


\vspace{-1mm}
\subsection{Analysis on Magnetic Distortion} \label{DBdesign}
% In this subsection, we introduce our observations on the nature of magnetic distortion, mainly from temporal and spatial aspects.
In this subsection, we study the nature of magnetic distortion, mainly from temporal and spatial aspects.
\vspace{-1mm}
% as support for our system design that models magnetic distortion.


\subsubsection{Temporal Stability}  \label{stability}
Geological magnetic fields are stable, and the artificial metal structures hardly move,  making the distortion pattern of the magnetic field almost constant. 
Figure \ref{temporal} shows the stability of a static magnetometer's readings in an indoor environment for 12 hours.
The three lines are the readings on the 3 axes of the magnetometer, which are relatively stable, despite the noise.
% Despite the noise, we can see the readings are relatively stable.
Several other works on magnetic fingerprinting also verify this chronological stability \cite{chung2011indoor,xie2014maloc,shao2016location,wang2021mvp}. 
% The work MVP \cite{wang2021mvp}, which uses magnetic fingerprints to locate vehicles in tunnels, confirms the stability of magnetic distortion pattern across years.
% Refer Refer Refer
In conclusion, in most cases, we can regard the magnetic field as a constant field.
\highlight{
This temporal stability verifies that it is possible to model the magnetic distortion at certain locations, and use it to assist the algorithm in the future when the device visits the same locations again.
% However, we do not specifically discuss extreme cases, such as drastic change in indoor magnetic environments that only happens if building structures significantly change.
}
% \begin{figure}
%     \centering
%     % \vspace{-2cm}
%     \includegraphics[width=0.54\linewidth]{fig/mobi_muse_devM.pdf}
%     \vspace{-0.1cm}
%    \caption{Orientation estimation error under different different distortion levels.}
%     \vspace{-0.5cm}
%     \label{muse_devM}
% \end{figure}





% \begin{figure}
%     \centering
%     % \vspace{-2cm}
%     \includegraphics[width=0.61\linewidth]{fig/mobi_dist.pdf}
%     \vspace{-0.1cm}
%    \caption{Distribution of distance between two nearby time steps (20ms).}
%     \vspace{-0.5cm}
%     \label{dist}
% \end{figure}
\vspace{-1mm}
\subsubsection{Spatial Correlation}\label{spatial corr}
% Since magnetic fields are not related with time, w
We then explore the spatial correlation of magnetic field.
% of different locations.
% Intuitively, the closer two locations are, the more similar their magnetic field should be.
As an example, we scan the magnetic field in a corridor.
We randomly sample a pair of locations $\overrightarrow{x_1}$ and $\overrightarrow{x_2}$ and measure their magnetic field directions $\overrightarrow{M}(\overrightarrow{x_1})$, $\overrightarrow{M}(\overrightarrow{x_2})$ , then we calculate the angular difference between the directions.
With a large amount of random pairs of $\overrightarrow{x_1}$ and $\overrightarrow{x_2}$, Figure \ref{spatial}\footnote{Theoretically, when the distance is near 0mm, the angular difference should also approach 0°, but not in Figure \ref{spatial}, which is possibly due to the sensor noise in the magnetometer.} shows the relationship between the magnetic field direction difference and the distance between $\overrightarrow{x_1}$ and $\overrightarrow{x_2}$. 
If the distance is limited, the difference of magnetic field directions is also limited.
This spatial correlation implies that we can model the distortion with certain spatial resolution.
\vspace{-1mm}
% Theoretically when the distance is near 0mm, the angular difference should also approach 0°, but not in Figure \ref{spatial}, which is possibly due to the sensor noise in the magnetometer.


==> Discuss_v2.tex <==
\section{Discussion}

\subsection{Supplementary Design I: Whether to Use Database in Distortion-Free Scenarios}\label{determine use or not}
In section \ref{pla}, we showed that database does not improve orientation estimation in some scenarios, where magnetic distortion is negligible.
It would be wise to turn off database and merely rely on CF+ to estimated orientation, otherwise it would negate the purpose of database to model distortion.
This would also reduce system complexity and save computation and memory resources.

Based on our experience and observation in magnetic distortion, we propose to use magnetic field intensity information to identify distortion-free scenarios.
Magnetic field intensity, $B$ reflects rich information on magnetic distortion, and can be convenient measured without know orientation.
Additionally we only request the time-serial magnetic field intensity measurement, which even do not require location information.
All measurement can be conveniently performed using a single magnetometer.
For smartphones, there are off-the-shelf application that can measure magnetic field intensity with integrated magnetometer.
Here we demonstrate two effective criteria to conveniently identify using on magnetic field intensity information, so that we can turn database off when it is not necessary.




\textbf{Criterion A: magnetic field intensity range.} 
Healthy, namely distortion-free magnetic fields usually have magnetic field intensity distribution from 45$\mu T$ to 55$\mu T$.
Thus if all intensity measurements are in the range of 40$\mu T$ to 60$\mu T$, criterion A is to be consider TRUE.

\textbf{Criterion B: magnetic field intensity relative variance.}
The relative variance of magnetic field intensity refers to $\frac{\sigma_B}{\overline{B}}$, the population deviation of $B$ divided by the expectation of $B$, which is a unit-free quantity describing how severe the intensity relatively changes.
Variance of intensity is usually greater in distorted magnetic fields.
If the relative variance in the area is smaller than 0.135, criterion B is to be considered TRUE.

We identify scenarios with $dev_M$<10° as distortion-free scenarios, and use the two criteria to recognize these scenarios among our data.
As table \ref{use_or_not} shows, the F1 score of criterion A is 94.12$\%$ and for B it is 91.74$\%$.
However if we combine A and B, we can have a F1 score of 96$\%$, as well as 96$\%$ precision and 96$\%$ recall.
As a conclusion, with the two criteria, we can conveniently and accurately identify distortion-free scenarios where database could be turned OFF to save computation and memory.

\begin{table}
    \centering
        \caption{Distortion-free scenario identification with two criteria.}
            \vspace{-0.1in}
    \begin{tabular}{|l|c|c|c|}
        \hline
          & Criterion A & Criterion B & Using both \\
        \hline
         Precision & 92.31$\%$ & 84.75$\%$ & 96.00$\%$ \\
         \hline
         Recall & 96.00$\%$ & 100$\%$ & 96.00$\%$ \\
         \hline
         F1 score & 94.12$\%$ & 91.74$\%$ & 96.00$\%$ \\
         \hline
    \end{tabular}
  \vspace{-0.2in}
    \label{use_or_not}
\end{table}


% \subsection{Supplementary Design II: Detecting and Emerging with Ambient History Databases}
% \label{merge2}
% Consider a user conducted arm motion tracking using \aliasSystem at a corner in the room.
% The second day, the user would like to do it again around the same corner.
% In such situation, it would be convenient for \aliasSystem to utilize the database$_1$ it built yesterday.
% However, database$_0$ was built within the GRF$_1$ that \aliasSystem initialized yesterday.
% Note this GRF$_0$ is not the actual global reference, instead it is only a global reference defined by \aliasSystem yesterday, using magnetometer measurement as 'front' and accelerometer measurement as 'down' (Section \ref{initialize}).
% When the user turns on the system again, \aliasSystem will have no idea where it is, nor which direction it is facing.

% Given that the initialization location of yesterday and today 
% % , $\overrightarrow{loc}_0$ and $\overrightarrow{loc}_1$ 
% could be different.
% In a distorted magnetic field, magnetometer could read differently at different locations, thus for the initialization, magnetometer could read different directions than yesterday, which further makes GRF$_1$ different than the GRF we are going to build today.
% This hinders \aliasSystem from knowing where GRF$_0$ is and which direction it is facing, let alone using the database$_1$ built in GRF$_0$.

% To make use of database$_0$, we propose an ambient history database detection and merging mechanism.
% It will verify the similarity between database$_0$ and database$_1$ by examining the difference of magnetic field intensity, with tentative compensations for the location and angular bias between GRF$_0$ and GRF$_1$.
% If the examined difference is consider below a certain threshold, it will merge database$_0$ onto database$_1$, thus accelerating the building process of database$_1$.

% At the beginning, We first let \aliasSystem start running without any information on GRF$_0$ or database$_0$.
% It initializes its own GRF$_1$ and builds a new database$_1$.
% When database$_1$ comes into an adequate size, we try to verify the similarity between database$_0$ and database$_1$. 
% We do not use the anchor directions in the database for this verification, for it is at the mercy of the error in the orientation input used to update the anchors, which is exactly the orientation estimation error.
% Instead we use the magnetic field intensity recorded along with the databases, mentioned in Section \ref{merge1}, which is more reliable in such verification.
% We sample in both database$_0$ and database$_1$, with a step length of $K_v\cdot l_{db}$ to verify the similarity, where $l_{db}$ is the database spatial resolution introduced Section \ref{resolution}, and $K_v$ is a integer ratio that controls the step length.
% For example, when $l_{db}$=10cm, $K_v$ is set to 3, so that we take one sample in every 30cm along X, Y, and Z axes, reducing the complexity for by 27x to save computation resource.

% Since database$_1$ is being built in a different GRF$_1$ than GRF$_0$, in which database$_0$ was built, we also need to apply different location bias (3-DoF) and rotations(3-DoF) onto database$_0$ to see if it matches with database$_1$.
% Fortunately, we know that GRF$_0$ and GRF$_1$ shares the same Z-axis, or the 'up' direction, so we only need to test the remaining 1-DoF rotation along Z-axis.
% Assume we have sampled the intensity at location $(x_1,y_1,z_1)$ of database$_1$ and wish to sample at the same physical location in database$_0$, then for every combination of 3-DoF location bias $(x_b,y_b,z_b)$ and 1-DoF Z-axis rotation $\theta_b$, we will sample at location $(x_0,y_0,z_0)$ in database$_0$, with:
% \begin{equation}
%     x_0 = x_1 \cdot cos(\theta_b) + y_1 \cdot sin(\theta_b) + x_b
%     \hspace{1cm}
%     y_0 = y_1 \cdot cos(\theta_b) - x_1 \cdot sin(\theta_b) + y_b
%     \hspace{1cm}
%     z_0 = z_1 + z_b
% \end{equation}

% We then test different combination of $(x_b,y_b,z_b)$ and $\theta_b$ to find the lowest average difference in the intensity.
% Figure~\ref{merge_theta} and \ref{merge_loc} depict how the intensity difference changes when we change the bias factors ($(x_b,y_b,z_b)$ and $\theta_b$). 
% The intensity difference decreases to almost 1 ${\mu}T$ when we find the best bias factors.
% % , we merge database$_1$ into database$_2$, so that the building process of database$_1$ is greatly propelled.

% We run the above verification every minute, and merge two databases if the average difference is lower than a certain threshold, e.g., 10$\%$ of the average magnetic field intensities in the surrounding.

% % This mechanism will not only speed up database construction in the presence of an existing database, but also in potential commercial application scenarios, if a high accuracy database had been prepared, \aliasSystem could then efficiently load that well prepared database and transform in to $MDR_D+$.

% % \begin{figure}
% %     \centering
% %     \vspace{-2cm}
% %     \includegraphics[width=0.6\textwidth]{fig/mobi_merge_theta.pdf}
% %     \vspace{-4cm}
% %    \caption{The examined magnetic intensity difference along $\theta_b$.}
% % \label{merge_theta}
% % \end{figure}

% \begin{figure}[tbp]
%     \begin{minipage}[t]{0.47\linewidth}
%         % \hspace{1cm}
%         % \vspace{-3cm}
%         \centering
%         \includegraphics[width=1\textwidth]{fig/mobi_merge_theta.pdf}
%         % \vspace{-3.5cm}
%         \caption{Examined intensity difference along $\theta_b$.}
%         \label{merge_theta}
%         % \vspace{-2cm}
%     \end{minipage}
%     % \hspace{0.1cm}
%     \begin{minipage}[t]{0.47\linewidth}
%         % \vspace{-3cm}
%         \centering
%         \includegraphics[width=1\textwidth]{fig/mobi_merge_loc.pdf}
%         % \vspace{-3.5cm}
%         \caption{Examined intensity difference along $x_b$, $y_b$, $z_b$.}
%         \label{merge_loc}
%         % \vspace{-2cm}
%     \end{minipage}
% \end{figure}



\subsection{Impact of Database Spatial Resolution}

We conduct real experiments to examine the impact of the spatial resolution of the database, $l_{db}$, introduced in Section \ref{resolution}.
Figure \ref{prec} shows the orientation error of \aliasSystem with different $l_{db}$.
$l_{db}$=10cm gives the best performance.
Either when $l_{db}$ is too large or too small, the performance deteriorates.
This demonstrates, $l_{db}$=10cm would be the best spatial resolution for \aliasSystem to model distortion with the database.
If the resolution is too fine, for example, $l_{db}$=0.025m, localization error would flood over the resolution causing the recorded anchors to be incorrect.
If the resolution is too coarse, for example, $l_{db}$=0.3m, the database would lose the ability to model distortion, due to the spatial correlation of magnetic field (Section \ref{spatial corr}).






% \subsection{Why not MUSE}

% As shown in Figure \ref{overall}, MUSE has an average orientation error of 29.57°, which is slightly higher than CF.
% This is possibly because MUSE's application scenario is slightly different from ours.
% While we focus on arm motion tracking, MUSE on the other hand tracked orientation in scenarios of health rehabilitation and basketball.
% As CF and MUSE both use magnetometer for calibration all the time, their major difference is the way they use accelerometer.
% CF always uses accelerometer, while MUSE use it only when the system is considered as static.
% MUSE set a threshold for acceleration magnitude to determine if the system is static.
% For example, if the measured magnitude of acceleration is within the range of $9.8\pm0.5m/s^2$, the system is considered as static.
% MUSE thinks only in such static moments, the accelerometer could be considered trustworthy.
% % so that via only using it in the static moments, it will improve the orientation estimation accuracy.
% However, we argue that, although MUSE improves the quality of the accelerometer usage via only using it in static moment, MUSE loses many opportunities to use accelerometer for calibration.
% With our collected data, we conduct real experiment on MUSE to support this argument.
% We tune the accelerometer quality via changing the threshold, which will also change the overall proportion of the moments that are considered static.
% Figure \ref{why not muse} shows the experiment results.
% In the moment that the system is considered static, as we widen the threshold, the angular error of accelerometer direction rises.
% However, also via widening the threshold, we gain much more effective static ratio, which means how much percentage of the total duration that the system could be consider static, and could use accelerometer for calibration.
% It quantifies the opportunities to use accelerometer.
% In this trade off, orientation error decreases as we widen the threshold.
% It means that the effective static ratio has a greater beneficial influence over the quality of accelerometer.
% When the ratio reaches 100$\%$, it means forever using accelerometer, which changes MUSE into CF.
% As a conclusion, the reason CF wins over MUSE in this application is that via sacrificing the accelerometer quality, while gaining valuable opportunities to use accelerometer for calibration.

\begin{figure}[htbp]
    \begin{minipage}[t]{0.47\linewidth}
        % \vspace{-3cm}
        \centering
        \includegraphics[width=1\textwidth]{fig/mobi_why_not_muse.pdf}
        % \vspace{-3.5cm}
        \caption{Orientation error of MUSE $\&$ effective static ratio, along the tuned accelerometer direction error at static moments.}
        \label{why not muse}
        % \vspace{-2cm}
    \end{minipage}
    % \hspace{0.5cm}
    \begin{minipage}[t]{0.47\linewidth}
        % \vspace{-3cm}
        \centering
        \includegraphics[width=1\textwidth]{fig/mobi_why_not_muse.pdf}
        % \vspace{-3.5cm}
        \caption{Orientation error of MUSE $\&$ effective static ratio, along the tuned accelerometer direction error at static moments.}
        \label{why not muse}
        % \vspace{-2cm}
    \end{minipage}
\end{figure}



% \subsection{Terminology Correction}
% The term "Magnetic Field Intensity", that we kept mentioning throughout the paper, actually refers to Magnetic Flux Intensity, usually denoted as $\overrightarrow{B}$.
% Its unit is $T$, Tesla.
% In physics, Magnetic Field Intensity actually 
% refers to $\overrightarrow{H}$, whose unit is $A/m$.
% The relationship between them is: $\overrightarrow{H}=\frac{\overrightarrow{B}}{\mu_0}-\overrightarrow{M}$.
% We simply used the term "Magnetic Field Intensity" for more intuitive expression.


\subsection{Error in Gravity Calibration}
% \begin{figure} 
%   \includegraphics[width=8cm]{fig/acc error.png}
%   \caption{Accelerometer direction error by linear acceleration}
%   \label{acc_error}
% \end{figure}
The error of accelerometer direction is the angle between $\overrightarrow{e_{acc}}$ and $\overrightarrow{anchor_G}$. 
We define this error as $err_G$, $err_G=arccos(\overrightarrow{e_{acc}}\cdot\overrightarrow{anchor_G})$.
The major error in $\overrightarrow{e_{acc}}$ comes from the influence of linear acceleration.
Additionally, $\overrightarrow{anchor_G}$ is absolutely (0,0,-1) and cannot have errors.
Thus we conclude the error in gravity calibration comes from \textbf{'calibrating a false $\overrightarrow{e_{acc}}$ with true $\overrightarrow{anchor_G}$'}.
Figure \ref{acc_error_2} shows the distribution of the amplitude of linear acceleration in daily arm movements. 
It ranges from 0 to around 4 m/s$^2$.
Figure \ref{acc_error} shows the relationship between $err_G$ and linear acceleration.
$err_G$ is limited by linear acceleration amplitude, and it is rare for $err_G$ to reach or exceed 20°.


\begin{figure}[htbp] %通栏
    \begin{minipage}[t]{0.47\linewidth}
        \centering
        % \vspace{-3cm}
        % \hspace{-2cm}
        \includegraphics[width=1\textwidth]{fig/mobi_acc_error_2.pdf}
        % \vspace{-3.6cm}
        \caption{CDF of linear acceleration amplitude}
        \label{acc_error_2}
    \end{minipage}
    % \hspace{0.5cm}
    \begin{minipage}[t]{0.47\linewidth}
        \centering
        % \vspace{-3cm}
        % \hspace{-2cm}
        \includegraphics[width=1\textwidth]{fig/mobi_acc_error.pdf}
        % \vspace{-3.6cm}
        \caption{Cross distribution of $err_G$ and linear acceleration}
        \label{acc_error}
    \end{minipage}
\end{figure}

%矢量图
\subsection{Comparison Between the Two Errors}
% We claim that the error from magnetic calibration is a great influence than gravity calibration.

\textbf{We invite 10 volunteers to collect daily movements at 10 places over 27 hours.}
Movements include pointing to objects in front, writing letters in the air and simple exercising.
The data traces are collected at different places to reflect the impact of magnetic distortion.
They are also collected at different arm motion speed and movement amplitude to reflect the impact of linear acceleration.
% Data traces are around 10min $\sim$ 20min.
% data in 12 locations with different magnetic environments, across 10 different buildings, with a total time length of .
Details on the data traces will be given in Section 5. 

\begin{figure}[htbp] %通栏
    \begin{minipage}[t]{0.47\linewidth}
        \centering
        % \vspace{-3cm}
        \includegraphics[width=\textwidth]{fig/mobi_GvsM2.pdf}
        % % \vspace{-3.6cm}
        \caption{CDF of $\frac{dev_M}{err_G}$ ratio}
        \label{GM1}
    \end{minipage}
    % \hspace{0.5cm}
    \begin{minipage}[t]{0.47\linewidth}
        \centering
        % \vspace{-3.3cm}
        % \hspace{-1cm}
        \includegraphics[width=0.9\textwidth]{fig/mobi_GvsM1.pdf}
        % \vspace{-3.96cm}
        \caption{Cross distribution of $err_G$ and $dev_M$}
        \label{GM2}
    \end{minipage}
\end{figure}

Figure \ref{GM2} shows the CDF of $\frac{dev_M}{err_G}$ ratio of all data traces. 
We can see in more than $59\%$ of the traces, $dev_M$ is greater than $err_G$, meaning magnetic calibration is making bigger trouble than gravity.
It shows the trouble of magnetic calibration is more pervasive than the trouble of gravity calibration.
Figure \ref{GM1} shows the distribution of average $err_G$ and $dev_M$ across all data traces. 
$dev_M$ spans from 0° to 60°+, while $err_G$ only spans from 0° to 25°.
It means the trouble of magnetic calibration is not only more pervasive, but also impacts greater.


Finally, to demonstrate the direct effect, we run CF under different $err_G$ and $dev_M$.
Figure \ref{CFM} and Figure \ref{CFG} show the experiment results, which are the aggregated results of multiple data traces.
    
    
Figure \ref{CFM} shows the performance of CF at different $dev_M$.
We can see, as $dev_M$ increases from 7° to 45°, CF orientation error increases from 20° to 40°, While in Figure \ref{CFG}, as $err_G$ increases from 6° to 20°, CF performance changes little.
The different range of X-axis of $dev_M$ and $err_G$ is because $dev_M$ does have larger range than $err_G$, corresponding to the distribution shown in Figure \ref{GM2}.
% Meanwhile $err_G$ has little effect on Gyro+Mag, due Gyro+Mag does not use magnetometer, except for the initialization process. Same for $dev_M$ to Gyro+Acc. 
% Gyro+Acc is even more sensitive to the variation of $err_G$, because accelerometer is the calibration for it. Same $dev_M$ to Gyro+mag.

Experiment implementation: 
We acquire the ground truth gravity direction in WRF via: $\overrightarrow{G}^{WRF}=[0,0,-1]\cdot\Theta_0^{-1}$. We then calculate a linear combination of ground truth gravity direction in WRF and an original accelerometer reading direction in WRF with a ratio $k_c$: $(1-k_c)\overrightarrow{e_{acc}^{WRF}}+k_c\cdot\overrightarrow{G}^{WRF}$.
We further normalize this new vector and finally overwrite the accelerometer reading direction in WRF with this normalized new vector, and feed it to CF as a simulated accelerometer input.
Thus by tuning ratio $k_c$, we can have different $err_G$ to simulate different accelerometer quality.
The same principle is used to tune $dev_M$.
We tune $err_G$ and $dev_M$ on the same set of data traces and generate variant data traces.
We let $0 \leq k_c \leq 1$ , so that it will only decrease $err_G$ and $dev_M$.


% A conclusion, magnetic calibration is the greatest bottleneck to be solved.



    % \textbf{CF}: Classical complementary filter with full sensors input.
    
    % \textbf{CF without Mag}: CF without magnetometer, meaning only using accelerometer to calibrate gyroscope integration.
    
    % \textbf{CF without Acc}: CF without magnetometer.
    
    % \textbf{Gyro only}: Only using gyroscope integration. 
    
    % \textbf{Calibration only}: Only using magnetometer and accelerometer could also provide orientation estimation, which is actually constantly performing initialization.

\begin{figure}[htbp] %通栏
    \begin{minipage}[t]{0.47\linewidth}
        \centering
        % \vspace{-3cm}
        \includegraphics[width=\textwidth]{fig/mobi_CF_M.pdf}
        % \vspace{-3.6cm}
        \caption{CF error under different $dev_M$, with and without magnetometer}
        \label{CFM}
    \end{minipage}
    % \hspace{0.5cm}
    \begin{minipage}[t]{0.47\linewidth}
        \centering
        % \vspace{-3cm}
        \includegraphics[width=\textwidth]{fig/mobi_CF_G.pdf}
        % \vspace{-3.6cm}
        \caption{CF error under different $err_G$, with and without magnetometer}
        \label{CFG}
    \end{minipage}
\end{figure}


\subsection{Do NOT Discard Magnetic Calibration}\label{gyro+acc}
Even though magnetic calibration brings CF big trouble, it is still unwise not to use it.
The other curve in Figure \ref{CFM} and Figure \ref{CFG}: 'Gyro+Acc' shows the error of CF without magnetometer, namely only using gyroscope and accelerometer.
Clearly it is far worse than CF under all circumstances.
% ############
This difference is due to the absence of magnetic calibration. 
Gyro+acc only has gravity providing a 2-DoF calibration, leaving 1 remaining direction without calibration. 
This direction is actually the direction of gravity itself, namely $\overrightarrow{anchor_G}$ or the Z-axis.
Accelerometer cannot detect any rotation along this direction, thus the gyroscope integration 'drift' will forever accumulate along this direction.

% ###########

% \begin{figure} 
%   \includegraphics[width=6cm]{fig/nomag.png}
%   \caption{Error of gyro+acc on Z-axis VS gyroscope only}
%   \label{nomag}
% \end{figure}

% To further demonstrate this issue, we separate and zoom in on the angular error along $\overrightarrow{e_z}$.
% Figure\ref{nomag} compares the angular error of gyro+acc on Z-axis with the error of the gyroscope-only method. 
% Despite an oscillation, we can see the error along $\overrightarrow{e_z}$ is growing almost at the same speed as gyro-only mode. 
% This 
% visualizes
% % gives a shocking scene on 
% what would happen if calibration is totally absent on one direction.
% Accelerometer does not make helpful contribution along this direction, thus leaving the error accumulating along $\overrightarrow{e_z}$. Orientation accuracy failure is only a matter of time.
% The reason we are seeing an oscillation in the error of gyro+acc on Z-axis is because accelerometer is vibrating around (0,0,-1), and may introduce a random rotation on Z-axis, but it will not help with the accuracy.
%(???????)

Magnetic anchor points to a different direction from gravity anchor, and thus is capable of calibrating that 1 remaining freedom.
As a conclusion, only with full sensor inputs, can we fully calibrate all 3-DoF and have stable orientation accuracy.
Thus we have no option but to face and solve the issue magnetic calibration.



==> Distortion_Free_Detection.tex <==
% FFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFF

\subsection{Distortion-Free Detection}\label{determine use or not}
% Based on the observations for magnetic distortion, 
If distortion hardly exists in a place, database will not help orientation estimation (to be verified in Section~\ref{pla}).
In order to save computation, we propose to use magnetic field magnitude information to identify distortion-free scenarios.
In a new place, \aliasSystem collects short magnetometer data to detect distortion.
If the place is detected as magnetic distortion-free, we turn off the database.
Magnetic field magnitude $M$ reflects rich information on magnetic distortion, and can be conveniently measured with magnetometer.
% Additionally we only request the time-serial magnetic field magnitude measurement, which even do not require location information.
% All measurement can be conveniently performed using a single magnetometer.
% For smartphones, there are off-the-shelf application that can measure magnetic field magnitude with integrated magnetometer.
% we two criteria to conveniently detect distortion-free places.
Using $M$, we design two criteria to detect the distortion-free places:

\begin{itemize} [leftmargin=*]
    \item \textbf{Criterion A:} 
    \textit{Range of $M$.}
    Distortion-free magnetic fields usually have an magnitude distribution from 45$\mu T$ to 55$\mu T$.
    If all magnitude measurements are in the range of 40$\mu T$ to 60$\mu T$, criterion A is considered true.
    Figure \ref{Criterion_A} shows the distribution of magnetic field magnitude of all data traces we collected, where the horizontal lines represent the range of magnetic field magnitude (left as minimum, right as maximum).
    We can see that when the range is not within 40$\mu T{\sim}60\mu T$, distortion tends to be high.
    There are also many lines that is in within 40$\mu T{\sim}60\mu T$, whose corresponding distortion is low (<10°).
    They overlap with each other and cannot be visualized clearly in Figure~\ref{Criterion_A}.
    
    \item \textbf{Criterion B:} 
    \textit{Variance of $M$.}
    The relative variance of magnetic field magnitude refers to $\frac{\sigma_M}{\overline{M}}$, namely the deviation of $M$ divided by the average of $M$, which describes how much the magnitude relatively changes.
    Magnitude variance is usually greater in distorted magnetic fields.
    If the relative variance in the area is smaller than 0.135, criterion B is considered true.
    Figure \ref{Criterion_B} shows the distribution of magnetic field magnitude variances of all data we collected.
    As the variance rises, distortion rises accordingly.
    
\end{itemize}
% 我把intensity改成magnitude，因为上下文都是magnitude. OK了
% We identify places with $dev_M$<10° as distortion-free, and 

When criteria A and B are both true, we consider a place to be distortion-free.
Detection accuracy will be evaluated in Section~\ref{detection_eval}.

\begin{figure}[tbp]
    \vspace{-2mm}
    \begin{minipage}[t]{0.45\linewidth}
        \centering
        \includegraphics[width=0.96\textwidth]{fig/sensys_A.pdf}
         \vspace{-3mm}
        \caption{Relationship between distortion and magnetic field magnitude.}
        % \vspace{0cm}
        \label{Criterion_A}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=0.9\textwidth]{fig/sensys_B.pdf}
         \vspace{-3mm}
        \caption{Relationship between the magnetic distortion and magnitude variance.}
        % \vspace{0cm}
        \label{Criterion_B}
    \end{minipage}
    \vspace{-2mm}
\end{figure}

% FFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFF


EVALUATION:


% FFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFF

\begin{table}
    \centering
    \vspace{1mm}
        \caption{Distortion-free scenario detection results.}
        \vspace{-4mm}
    \begin{tabular}{|l|c|c|c|}
        \hline
          & Criterion A & Criterion B & Using both \\
        \hline
         Precision & 92.31$\%$ & 84.75$\%$ & 96.00$\%$ \\
         \hline
         Recall & 96.00$\%$ & 100$\%$ & 96.00$\%$ \\
         \hline
         F1 score & 94.12$\%$ & 91.74$\%$ & 96.00$\%$ \\
         \hline
    \end{tabular}
  \vspace{-6mm}
    \label{use_or_not}
\end{table}

% FFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFF


\subsection{Distortion-Free Detection Accuracy}
\label{detection_eval}
We can avoid wasting computation by using the two criteria A and B designed in Section \ref{determine use or not} to recognize the magnetic distortion free scenarios and turn off the database in these scenarios.
To evaluate the effectiveness of these two criteria, we identify scenarios with distortion magnitude lower than 10° as distortion-free.

\balance

As table \ref{use_or_not} shows, F1 score of criterion A is 94.12$\%$, and for B is 91.74$\%$.
If we combine A and B, we have a F1 score of 96$\%$, as well as 96$\%$ precision and 96$\%$ recall.
As a conclusion, with the two criteria, we can conveniently and accurately identify distortion-free scenarios where database could be turned off to save computation.

According to our distortion-free criteria, among the 10 places in Table \ref{places}, only three places are distortion-free: 'Conference room', 'Outdoor' and \ 'House'.
It validates that magnetic distortion commonly exists in buildings.
% where \aliasSystem provides significant performance gain in orientation estimation.
As shown in the column on the right of Table \ref{places}, enabling the database in 'Outdoor' only grants 3.43$\%$ accuracy boost, and for 'House', it is only 4.37$\%$.
However, in 'Conference room', the database will decrease the accuracy by 1.83$\%$, due to potential database error.
If we turn off the database in these places, especially 'Conference room', we can save computation, while not affecting orientation accuracy much.
According to Table \ref{latency} in Section \ref{computation latency}, we can save 89.95$\%$ of the computation, since database is not needed, along with particle filter that serves the database.


\begin{figure}
    \centering
    \includegraphics{fig/bu}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}


% FFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFF
% System Design Overview:

\textbf{Distortion-free detection} (\textit{Section \ref{determine use or not}})\textbf{:}
We design two criteria for \aliasSystem to detect distortion-free places, and turn off the database if distortion is weak or absent, in order to save computation.
% FFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFFF

==> Imple.tex <==
\section{Implementation}
We used MATLAB for all experiments.
The PC is equipped with Intel Core i7-8750H CPU 2.20 GHz.


==> Intro_Error_Reduction_Old.tex <==
\textbf{\textcircled{1} For better accelerometer calibration accuracy, MUSE \cite{muse} and $A^3$ \cite{A3} perform accelerometer calibration only when the system is static, namely when accelerometer measures roughly 9.8m/s$^2$.
Instead, we argue to loosen that restriction to gain more calibration opportunities and provide more effective suppression on the gyroscope drift.
The sacrifice is a decrease in accelerometer calibration accuracy.
Therefore, through extensive experiments, we find the optimal balance between accuracy and opportunity for accelerometer calibration, by setting \textit{'accelerometer measures 9.8$\pm$1.3m/s$^2$'} as calibration condition, and reaches lowest orientation error.}
% 1) We conduct extensive experiments and find that although the accelerometer's reading is not perfectly the gravitational acceleration, the linear acceleration caused by arm movement sometimes is limited. 
% In these situations, the accelerometer's readings can still provide useful information for calibrating the orientation tracking results of the gyroscope. 
% Therefore, different from MUSE \cite{muse} and $A^3$ \cite{A3}, we loosen the requirement for accelerometer calibration, to gain more calibration opportunities, providing more effective suppression on the gyroscope drift. 
%XXXXXXXXX
% 1) We refine the usage of accelerometer in orientation estimation, even when the arm is not static. %XXXXXXXXXX
% It is different from prior work \cite{muse} that only uses magnetometer. 
% 没有moving constantly一说
\textbf{\textcircled{2} }
% Also in orientation estimation via complementary filter, 
\textbf{We find that in existing works, accelerometer and magnetometer calibrations and gyroscope integration all share the same iteration frequency (50Hz, based on our smartwatch sampling rate).
As a result accelerometer and magnetometer are constantly calibrating high-accuracy gyroscope integration result, with their low-accuracy readings, thus decreasing overall orientation performance.
Therefore, based on experiments on 70 one-minute data traces, we find the best frequency for accelerometer and magnetometer calibrations, so that they calibrate orientation result only when gyroscope drift is high enough, so that calibration could deliver positive effect.}
 % The above techniques improve orientation accuracy, which further improves database operations.
% Better database operations will in return improve orientation estimation.
% resulting in an even larger improvement than the direct improvement.
\textbf{In summary, the above two techniques improve orientation accuracy, which further improves database operations; and better database operations will in return improve orientation estimation.}
% we tune the frequency for the usage of the magnetometer and accelerometer to better adapt to their noisy nature.
% LLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLL
\textbf{\textcircled{3} In localization via particle filter, acceleration is calculated via dividing location difference twice ($a=\frac{\Delta x}{\Delta t^2}$). 
However, we find that, the short calculation interval (20ms for 50Hz) will enlarge error in location by a ratio of $\frac{1}{(20ms)^2}=2500s^{-2}$, thus causing an acceleration anticipation issue.
To that end, we increase the interval of particle filter iteration, in order to decrease the error enlarging ratio.
We conduct experiment and find that the best interval is 100ms.
Next, in order to maintain particle filter's cooperation with the database and complementary filter, which are still functioning with an interval of 20ms, we design an interpolation strategy to fill the missing location inferences.}
% LLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLL


==> Intro_deadlock_old.tex <==
% The query of magnetic profiling database for orientation estimation, we need the watch's current location.
% Meanwhile, to infer the watch's location using IMU sensors, we need its orientation as input. 
However, to infer the watch's location, we need orientation as input, which forms a deadlock. 
% To solve this deadlock problem, we test two location methods for database query, i.e., the location measured at last time step, and the location measured by the conventional particle filter method without using the database.
% To solve this deadlock problem, a naive solution is to estimate orientation without information from database, and then perform localization to query the database.
% After that it runs orientation estimation again.
% This solution is inefficient, since it runs orientation estimation twice, as well as inaccurate, since the first orientation is estimated without the help from
To solve that, a naive but inefficient way is to infer orientation without querying database, and then estimate location, so that it can finally query the database and estimate orientation again.
Instead, we leverage the continuity of human arm motion to solve the deadlock.
Based on real arm motion data we collect, we find that the speed of arm motion is limited (usually <1m/s), as well as the location difference between two time steps (usually <2cm).
% Therefore we come up with a solution for the deadlock that uses the location inferred from the previous time step to query the database.
Therefore, we use the location inferred from the previous time step to query the database, and thus solve the deadlock.
Experiments show that the continuity-solution outperforms the naive one, and thus we adopt the continuity-solution for \aliasSystem. 
% another baseline that insists on using current location information to query the database via sacrificing efficiency, and find that the former solution
% We conduct extensive experiment with 12 volunteers to compare this solution another naive solution that queries the database using location inferred at current time step, using orientation estimated without database information.
% [METHOD 1  METHOD 2]
% We conduct extensive experiments with 12 volunteers and quantify the location errors of these two methods. 
% Experiment results show that the first method provide higher accuracy since human's arm movement between two time steps (20 ms) is limited. 

==> Ktable.tex <==
\begin{table}
    \centering 
        \caption{Complementary filter error with different integration frequencies $K_{g}$ and calibration frequencies $K_{c}$.}
    \vspace{-0.1in}
    \begin{tabular}{|l|c|c|c|c|c|c|c}
        \hline
        \diagbox{$K_{c}$}{$K_{g}$} & $K_{g}$ = 1 & $K_{g}$ = 2 & $K_{g}$ = 3 & $K_{g}$ = 4 & $K_{g}$ = 5 \\%7 \\%& 10 \\
        \hline
% 50Hz 
$K_{c}$ = 1 & 21.82° & 21.84° & 21.87° & 21.93° & 22.12° \\
% 21.82 	21.84 	21.87 	21.93 	22.12 	23.13 
        \hline
% 25Hz 
$K_{c}$ = 2 & 20.60° & 20.62° & 20.70° & 20.72° & 20.96° \\
% 20.60 	20.62 	20.70 	20.72 	20.96 	22.54 
        \hline
% 16.67Hz
$K_{c}$ = 3 & 19.69° & 19.81° & 19.85° & 19.98° & 20.25° \\
% 19.69 	19.81 	19.85 	19.98 	20.25 	22.32 
        \hline
% 10Hz
$K_{c}$ = 5 & 18.50° & 18.51° & 18.61° & 18.62° & 18.81° \\
% 18.50 	18.51 	18.62 	18.81 	19.10 	21.15 
        \hline
% 5Hz
$K_{c}$ = 10 & 16.09° & 16.16° & 16.34° & 16.56° & 16.65° \\
% 16.09 	16.16 	16.34 	16.65 	17.43 	24.04 
        \hline
% 3.33Hz 
$K_{c}$ = 15 & 14.57° & 14.74° & 15.00° & 15.28° & 15.43° \\
% 14.57 	14.74 	15.00 	15.28 	17.75 	26.69 
        \hline
% 2.5Hz 
$K_{c}$ = 20 & 13.64° & 13.66° & 13.94° & 14.25° & 14.56° \\
% 13.63 	13.64 	13.94 	14.25 	18.84 	28.08
        \hline
% 2.27Hz 
$K_{c}$ = 22 & 13.63° & 13.66° & 13.93° & 14.24° & 14.85° \\
% 13.63 	13.66 	13.93 	14.24 	18.93 	29.12
        \hline
% 2.08Hz 

$K_{c}$ = 23 & 13.58° & 13.67° & 13.82° & 14.08° & 14.73° \\
%18.93° \\% & 29.12 \\
        \hline
  
$K_{c}$ = 24 & \textbf{13.26°} & 13.45° & 13.57° & 13.74° & 14.41° \\
% 13.26 	13.45 	13.57 	13.74 	18.77 	29.80 
        \hline
% 2Hz 
$K_{c}$ = 25 & 13.43° & 13.63° & 13.71° & 13.88° & 14.42° \\
% 13.43 	13.63 	13.71 	13.88 	18.84 	29.86 
        \hline
% 1.92Hz 
$K_{c}$ = 26 & 13.50° & 13.67° & 13.83° & 13.93° & 14.51° \\
% 13.50 	13.57 	13.63 	13.83 	19.22 	30.70 
        \hline
% 1.79Hz 
$K_{c}$ = 28 & 13.72° & 13.84° & 14.02° & 14.04° & 14.50° \\
% 13.72 	13.84 	14.02 	14.04 	20.04 	30.92 
        \hline
% 1.67Hz 
$K_{c}$ = 30 & 13.75° & 13.83° & 13.99° & 14.04° & 14.66° \\
% 13.75 	13.83 	13.99 	14.04 	19.99 	31.81 
        \hline
% 1.25Hz 
$K_{c}$ = 40 & 14.27° & 14.41° & 14.57° & 14.75° & 15.11° \\
% 14.27 	14.41 	14.57 	14.75 	22.06 	34.47 
        \hline
% 1Hz 
$K_{c}$ = 50 & 15.38° & 15.41° & 15.54° & 15.82° & 16.53° \\
% 15.38 	15.41 	15.54 	15.82 	25.47 	37.35 
        \hline
% 0.87Hz 
$K_{c}$ = 60 & 16.20° & 16.30° & 16.33° & 16.71° & 17.50° \\
% 16.20 	16.30 	16.33 	16.71 	26.59 	40.13 
         \hline
    \end{tabular}
    \vspace{-0.1in}

    \label{kk}
\end{table}

==> Loc_pro.tex <==
% 原本是第二个Design Section，也就是Error Reduction （Pro）Section的第三个subsection：
% \appendix

\vspace{-1mm}
\subsection{Corrected Acceleration Anticipation in Location Estimation}
\vspace{-1mm}
\label{secCorrectedPF}

\begin{figure*}[h]
    % \vspace{-3mm}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        % \vspace{-2.8cm}
        \centering
        \includegraphics[width=\textwidth]{fig/mobi_k_pf_acc.pdf}
        \vspace{-7mm}
        \caption{Distribution of acceleration anticipation with $K_{pf}=1$ and $K_{pf}=5$.}
        \label{linacc}
        % \vspace{-2cm}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.24\linewidth}
        % \vspace{-2.8cm}
        \centering
        \includegraphics[width=\textwidth]{fig/sensys_k_pf.pdf}
        \vspace{-7mm}
        \caption{Location error of particle filter with different $K_{pf}$ setting.}
        \label{Kpf}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=1\textwidth]{fig/interp.pdf}
        \vspace{-7mm}
        \caption{Example of linear interpolation using recent location results.}
        \label{interp}
        % \vspace{-2cm}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=1\textwidth]{fig/intuit.pdf}
        \vspace{-7mm}
        \caption{Example of intersection between interpolation and ground truth.}
        \label{intuit}
        % \vspace{-2cm}
    \end{minipage}
    \Description[bruh]{bruh bruh}
    \hfill
    \vspace{-3mm}
\end{figure*}


% As shown in Figure \ref{flow}, location information will be used both in the updating process and query process of the database.
% We also improve the accuracy of location estimation by enlarging the sampling interval of particle filter.
% We also improve location estimation by correcting inaccurately anticipated acceleration in particle filter.
In particle filter, each particle records the last three historical locations, which forms a temporal trajectory.
Based on the trajectory, particle filter calculates the velocity and acceleration of each particle, as shown in Equation \ref{pfacc}:



% \subsubsection{}

\vspace{-4.5mm}
\begin{equation}
    \begin{split} \label{pfacc}
        \overrightarrow{a}
        =\frac{\overrightarrow{v}(t+\frac{1}{2}\Delta t)-\overrightarrow{v}(t-\frac{1}{2}\Delta t)}{\Delta t}
        \\
        =\frac{\frac{(\overrightarrow{x}(t+\Delta t)-\overrightarrow{x}(t))}{\Delta t}-\frac{(\overrightarrow{x}(t)-\overrightarrow{x}(t-\Delta t))}{\Delta t}}{\Delta t}
        \\
        =\frac{\overrightarrow{x}(t+\Delta t)-2
        % \cdot 
        \overrightarrow{x}(t)+\overrightarrow{x}(t-\Delta t)}{\Delta t^2}
    \end{split}
\end{equation}
\vspace{-2.5mm}

When the particle filter anticipates this acceleration, the location difference: $\overrightarrow{loc}(t+\Delta t)-2\overrightarrow{loc}(t)+\overrightarrow{loc}(t-\Delta t)$, will be divided by $\Delta t^2$.
Given our smartwatch's default sampling interval $\Delta t=20ms$, then $\frac{1}{\Delta t^2}=2500s^{-2}$.
It will enlarge any location error by a ratio of $2500s^{-2}$.
We monitor the anticipated acceleration in particle filter and find it largely exceeds the limit of human motion, as "$K_{pf}$=1" in Figure \ref{linacc} shows the CDF of the anticipated acceleration
of all particles.
% An acceleration anticipation as high as 
$1000m/s^2$ is surreal for human and will result in inaccurate location estimation.





% \subsubsection{Solution} 
To correct this surreal anticipation, we enlarge the iteration interval $\Delta t$ to decrease $\frac{1}{\Delta t^2}$.
Instead of 20ms, we let particle filter run once in every $K_{pf} \cdot $ 20ms.
With real data of more than one hour, we evaluate particle filter's average location error with different $K_{pf}$, as shown in Figure \ref{Kpf}.
When $K_{pf}$=1, the location error is 0.1215m, which decreases to 0.1162m (by 4.36$\%$) as $K_{pf}$ increases to 5, because lower longer interval will have lower location error enlarging rate: $\frac{1}{(100ms)^2}=100s^{-2}$.
% Figure \ref{linacc} also shows the distribution of anticipated acceleration when $K_{pf}=5$, which is  $K_{pf}=1$.
% When $K_{pf}$=5, the result is 0.1361m, decreased by 4.33$\%$ than $K_{pf}$=1. 
When $K_{pf}>5$, location error increases, since particle filter do not have enough time resolution to track the motion.
% insufficient frequency is too low, 
% In the extreme case, if $K_{pf}=+\infty$, particle filter will stop working.
% , so that as $\Delta t$ grows larger, the error enlarging rate will be lower.
% However the frequency should also not be too low, otherwise particle filter will not be able to trace the motion with enough time resolution.
% E.g., if $\Delta t=100ms$, the enlarging rate will be $100s^{-2}$, 25 times smaller. 
The enlarged interval allows the motion signal in a longer period to be aggregated, outweighing noise in measurements.
Coincidentally, MUSE \cite{muse} also proposes to aggregate every five rounds for particle filter, but their purpose is to decrease computation latency, while we set $K_{pf}=5$ for higher location estimation accuracy, thus reduce location error in both query and updating process.




\textbf{Filling Enlarged Time Interval.}  
In Section \ref{deadlock}, to solve the deadlock problem, we proposed to use the location result from the previous step for database query.
% lowered the calculation frequency of particle filter by 5$\times$, we also increased the time interval between two steps with available location information by 5$\times$.
% According to figure \ref{dist}, most distances between two localized steps are below 10mm.
However, in achieving the best location result, we increased the particle filter calculation interval from 20ms to 100ms, while orientation estimation and the database components are still operating with a constant interval of 20ms. 
% With 100ms, the arm moves a longer distance, which will make the location result of the last time step further away from the current location of the watch.
Therefore, after every inference, there are four ($\frac{100ms}{20ms}-1$) blank steps to fill, in order to support database updating.
% maintain cooperation with other components.
To fill these gaps, a naive solution is to use the latest location results.
However, we further propose a linear interpolation strategy using the inferred locations to fill the blank time steps, which turns out to be more accurate.
As an intuitive example, in Figure \ref{interp}, for a blank step $t$, we interpolate its location result $\overrightarrow{x}(t)$ as the linear combination of the last two inferred locations $\overrightarrow{x}(t_1)$ and $\overrightarrow{x}(t_2)$:

% \vspace{-4.5mm}
\vspace{-3mm}
\begin{equation} \label{interp_equation}
    \overrightarrow{x}(t)
    =
    \frac{
        \overrightarrow{x}(t_2)
        \cdot
        (t-t_1)
        -
        \overrightarrow{x}(t_1) 
        \cdot 
        (t-t_2) 
    }
    {
        t_2-t_1
    }
    \hspace{0.33cm}
    (t_1 < t_2 < t)
\end{equation}
\vspace{-3mm}
% \vspace{-1.5mm}

 % focuses on one axis of the location vector, and gives an intuitive example of location interpolation.
% According to experimental results, for locations inferred by particle filter with $K_{pf}=5$, the average error is 0.1361m. %0.0965
We test the naive solution and the interpolation solution on all data traces.
% and calculate their accuracy.
Experiments show the naive solution has an average error of 0.1185m. %0.1384m. % 0.0981
The linear interpolation method, as introduced in Equation \ref{interp_equation}, has an average error of 0.1083m, which is even below the error of original estimation error of 0.1157m ($K_{pf}=5$, with blank steps). 
% 0.1268m
%8.99cm

To explain this, we first focus on one axis of the location vector, for example the X-axis.
As an intuitive example shown in Figure \ref{intuit}, the estimated location curve occasionally intersects with the ground truth curve.
 % also focuses on one axis of location vector, and provides an intuitive picture of this intersection, where 
At step $t_1$, estimated result > ground truth, while at step $t_2$, estimated result < ground truth.
Therefore the two curves intersect at some point between step $t_1$ and step $t_2$.
Around the intersection, interpolated results will approach the ground truth.
Dotted vertical lines in Figure \ref{intuit} represent the distance between interpolated results and the ground truth, which are shorter nearby the intersection, meaning error decreases in this area.
For other intervals, where the interpolation curve does intersect with the ground truth (e.g., between $t_2$ and $t_3$ in Figure \ref{intuit}), the error does not change much, compared to the original error.
% It forms a hourglass shape around the intersection, 
Statistics show that intersections take up to around 30$\%$ of the total time steps.
Specifically, for X, Y and Z axes, the statistics are 29.29$\%$, 29.83$\%$ and 30,68$\%$.




% \subsubsection{Longer Absence}
% Since we decreased the calculation frequency of particle filter, we would face a longer absence of location information, as we pre-alerted in \ref{absence}.
% If we still stick to the very last location result, due to the longer interval, query error and 
% To make up for this issue, we perform linear-interpolation to fill the absence with the sparse location results:

% \begin{equation}
%     \overrightarrow{loc}_{t+\Delta t}=((\Delta t+K_{pf}\Delta t)\overrightarrow{loc}_{t}-K_{pf}\Delta t\overrightarrow{loc}_{t-K_{pf}\Delta t})/(K_{pf}\cdot \Delta t)
% \end{equation}

% LLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLL

% 原本在introduction的段落：
% \textcircled{3} In location estimation via particle filter, acceleration is calculated via dividing location difference twice ($a=\frac{\Delta x}{\Delta t^2}$). 
% However, we find that, the short calculation interval (20ms for 50Hz) will enlarge error in location by a ratio of $\frac{1}{(20ms)^2}=2500s^{-2}$, thus causing an acceleration anticipation issue.
% To that end, we increase the interval of particle filter iteration, in order to decrease the error enlarging ratio.
% We conduct experiment and find that the best interval is 100ms.
% Next, in order to maintain particle filter's cooperation with the database and complementary filter, which are still functioning with an interval of 20ms, we design an interpolation strategy to fill the missing location inferences.



% LLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLL

% 原本是 Error Reduction 章节的Overview里的：

% Last, in location estimation via particle filter, we solve a false acceleration anticipation problem to improve location accuracy (\textit{Section \ref{secCorrectedPF}}).



% LLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLL

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> Pro.tex <==
% \appendix


\vspace{-1mm}
\section{Reducing Errors in Database Operations}\label{pro}
\vspace{-1mm}
% First thing first, we are not simply improving orientation and localization to achieve better performance, but also seeking to improve the usage of database with better orientation and location accuracy.
% In this section, we reduce errors in database query and updating.
% Database mainly performs updating and query.
% \textbf{Query Error:} 
As shown in Figure~\ref{flow}, database query relies on the estimated location as index.
Inaccurate query location leads to incorrect magnetic anchor, which then leads to wrong orientation estimation.
% \textbf{Updating Error:}
Moreover, database updating requires estimated orientation and location, while orientation and location errors will result in inaccurate datapoints.
% namely false anchors stored at incorrect locations.
% Errors in updating and query iteratively magnify each other as the workflow of \aliasSystem repeats.
% Late but not least, errors in updating and query iteratively magnify each other as the workflow of \aliasSystem repeats.
% The anchor will be further used by complementary filter to estimate orientation, which will then be used by particle filter to estimate location.

% XXXXXXXXXXXXXXXXXXXXXXXXXXXXX
% If we improve the accuracy of orientation and location estimations, they would lead to better database updating, and then more accurate query.
% If we could improve the accuracy of orientation, it would lead to better location estimation, since particle filter takes orientation to infer location.
If we could improve the accuracy of orientation and location, it would then improve the accuracy of database updating and query, which in return would improve orientation and location accuracy.
% As the workflow of \aliasSystem repeats, updating and query iteratively improve each other.
As the workflow of \aliasSystem repeats, the components would iteratively improve each other.
% Therefore, we expect an overall improvement of the final orientation estimation that is greater than the direct improvement in orientation estimation and localization.
Therefore, we expect an overall improvement in the final orientation accuracy that is greater than the direct improvement.
We first improve orientation estimation via finding the balance between quality and opportunity for accelerometer calibration (\textit{Section \ref{boost_ori_1}}).
Second, to avoid harmful calibrations, we reduce the frequencies for magnetometer and acceleration calibrations, so that they are performed only when they can improve orientation estimation (\textit{Section \ref{boost_ori_2}}).
Last, in location estimation via particle filter, we solve an inaccurate acceleration anticipation problem to improve location accuracy (\textit{Section \ref{secCorrectedPF}}).
\vspace{-1mm}
% make complementary filter better adapt to the noisy property of magnetic calibration and acceleration calibration




% LLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLL
% Last, in localization via particle filter, we solve a false acceleration anticipation problem to improve localization accuracy (\textit{Section \ref{secCorrectedPF}}).
% LLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLLL






% We then try to improve orientation accuracy via making complementary filter better adapt to the noisy property of the  calibrators.
% We also provide a refined strategy to determine whether to use accelerometer.
% Last, We solve a linear acceleration calculation problem within particle filter to improve localization.
% % the reason we try to improve orientation and localization is not only to directly improve them, but more importantly, 
% We will show by improving orientation and localization, we improved the input of database updating, and thus arrives at a even better performance than the direct improvement of orientation and localization.
% We name the upgraded system \aliasSystem.

% XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX

% \subsection{Error Tracing in Database Operations}
% \label{secErrorTracing}
% % Figure \ref{flow} gives an intuitive picture on how the error flows in \aliasSystem.

% The magnetometer is also used in the updating process, which can be improved via substituting it with magnetometers of higher quality.
% However, we do not discuss such potential in this paper.
% % We 
% therefore try to improve orientation and localization, for better usage of the database and we 
% expect to see a \textit{'1+1>2'} result.\label{1+1}

% \begin{figure} 
%     \centering
%     \vspace{-3cm}
%     \includegraphics[width=0.5\textwidth]{fig/mobi_gyro_cali.pdf}
%     \vspace{-3.5cm}
%     \caption{Visualized error accumulation of gyroscope integration VS errors of two calibration.}
%      \vspace{-0.5cm}
%     \label{gyrocali}
% \end{figure}


% \subsection{Improving Orientation Estimation to Refine Database Operations[DELETE]}
% Upgrading complementary filter via adapting to 'long-term' accuracy of calibrators
% Orientation will be used by database in the updating process to generate a datapoint, as shown in Figure \ref{flow}.
% In this section, we improve orientation estimation by making complementary filter better adapt to the noisy property of the calibrators, as well as proposing an improved strategy of accelerometer usage, based on MUSE \cite{muse} and $A^3$ \cite{A3}.



\vspace{-1mm}
\subsection{Preserving Opportunities for Accelerometer Calibration}  \label{boost_ori_1}
\vspace{-1mm}
% \subsection{Refined Accelerometer Usage: 9.799m/s$^2$?}

% \begin{figure} [tbp]
%     \begin{minipage}[t]{0.39\linewidth}
%         \vspace{-2mm}
%         \centering
%         \includegraphics[width=.92\linewidth]{fig/mobi_why_not_muse_1.pdf}
%         \vspace{-3mm}
%         \caption{Direction errors of accelerometer under different static boundary sizes.}
%         \label{why not muse 1}
%         % \vspace{-2cm}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[t]{0.55\linewidth}
%         \vspace{-2mm}
%         \centering
%         \includegraphics[width=.9\linewidth]{fig/mobi_why_not_muse_2.pdf}
%         \vspace{-3mm}
%         \caption{Orientation error in static opportunities $\&$ static opportunity proportion, along the static boundary size.}
%         \label{why not muse 2}
%     \end{minipage}
%     \vspace{-5mm}
% \end{figure}



% \begin{figure}
%     \centering
%     % \vspace{-2cm}
%     \includegraphics[width=0.7\linewidth]{fig/mobi_gyro_cali.pdf}
%     \vspace{-0.1cm}
%    \caption{Errors of gyroscope integration and calibrations.}
%     \vspace{-0.5cm}
%     \label{gyrocali}
% \end{figure}
MUSE~\cite{muse} and $A^3$~\cite{A3} opportunistically use accelerometer when the system is static.
They detect these opportunities when the accelerometer measurements are within a static boundary around $9.8m/s^2$, e.g., $9.8 \pm 0.3 m/s^2$.
% The latest work, MUSE, performs accelerometer calibration using a complementary filter. [?]
% Based on this mechanism, we 
% As shown in Figure \ref{overall}, MUSE has an average orientation error of 29.57°, which is slightly higher than complementary filter.
% This is possibly because MUSE's application scenario is slightly different from ours.
% While we focus on arm motion tracking, MUSE on the other hand tracked orientation in scenarios of health rehabilitation and basketball.
% As complementary filter and MUSE both use magnetometer for calibration all the time, their major difference is the way they use accelerometer.
% complementary filter always uses accelerometer, while MUSE use it only when the system is considered as static.
% MUSE set a boundary for acceleration magnitude to determine if the system is static.
% For example, if the measured magnitude of acceleration is within the range of $9.8\pm0.5m/s^2$, the system is considered as static.
% MUSE thinks only in such static moments, the accelerometer could be considered trustworthy.
% so that via only using it in the static moments, it will improve the orientation estimation accuracy.
Using one-hour arm motion data, we first examine the error of accelerometer direction during static opportunities, with different static boundary sizes. 
This error is calculated using the same principle as we calculate distortion magnitude: transforming accelerometer reading into GRF using ground truth orientation, and then compare it with gravity anchor.
As shown in Figure \ref{why not muse 1}, accelerometer is more trustworthy when the boundary is smaller.
However, if the boundary is too low ($<0.2m/s^2$), no time steps will be recognized as static opportunities.
% The average direction error can hardly decrease to zero, because the accelerometer sometimes may also measure roughly $9.8m/s^2$, but has a different direction from gravity.
As the boundary loosens, the direction error of accelerometer rises accordingly, and is capped at 6.13°.



We further test MUSE's performance with different static boundary sizes.
As shown in Figure \ref{why not muse 2} (Y axis on the left), surprisingly, MUSE's error is relatively high when the static boundary is limited (22.01° when the static boundary is $0.3m/s^2$, 22.57° for $0.2m/s^2$), despite that the accelerometer quality is high during the static opportunities.
To explain that, we argue that MUSE loses valuable calibration opportunities by restricting accelerometer usage.
We calculate the static opportunity proportion, namely the percentage of the time steps that are regarded as static opportunities, which is also shown in Figure \ref{why not muse 2} (Y axis on the right).
If the static boundary size is limited, the overall static opportunity proportion is low.
Without sufficient calibrations by accelerometer, magnetometer works alone to suppress the drift of gyroscope integration.
On top of that, the drift along the direction of magnetometer reading direction cannot be calibrated by magnetometer itself.
% In the extreme case, if the static boundary is zero, meaning accelerometer is totally disabled, the


We find that as the static boundary loosens ($<1.3m/s^2$), the static opportunity proportion largely increases, which also results in an improvement of MUSE's performance.
This is due to higher frequency of accelerometer usage.
However, when the static boundary is too large, time steps that have low accelerometer accuracy may also be considered as static opportunities, thus increasing the error of MUSE.
As shown in Figure \ref{why not muse 2}, frequency and quality of calibration reach the balance when the static boundary is $1.3m/s^2$ and the static opportunities proportion is $75\%$, then the orientation error arrives at its minimum, 19.98°, 9.22$\%$ lower than when the static boundary is $0.3m/s^2$.
As a conclusion, based on MUSE, we further propose to use accelerometer not only when the system is static, but also when the system is nearly static, for example $9.8 \pm 1.3m/s^2$, so that accelerometer calibrations maintain both sufficient frequency and quality.
We then adopt this strategy for the complementary filter in \aliasSystem.
\vspace{-1mm}

% We tune the accelerometer quality via changing the static boundary, which will also change the overall proportion of the moments that are considered static.
% Figure \ref{why not muse} shows the experiment results.
% In the moment that the system is considered static, as we widen the static boundary, the angular error of accelerometer direction rises.
% However, also via widening the static boundary, we gain much more effective static ratio, which means how much percentage of the total duration that the system could be consider static, and could use accelerometer for calibration.
% It quantifies the opportunities to use accelerometer.
% In this trade off, orientation error decreases as we widen the static boundary.
% It means that the effective static ratio has a greater beneficial influence over the quality of accelerometer.
% When the ratio reaches 100$\%$, it means forever using accelerometer, which changes MUSE into complementary filter.
% As a conclusion, the reason complementary filter wins over MUSE in this application is that via sacrificing the accelerometer quality, while gaining valuable opportunities to use accelerometer for calibration.

% \begin{figure}
%     \centering
%     \hspace{-0.3cm}
%     \vspace{-0.2cm}
%     \includegraphics[width=0.72\linewidth]{fig/mobi_gyro_cali.pdf}
%     \vspace{-2mm}
%    \caption{Angular errors of gyroscope integration, accelerometer, and magnetometer.}
%     \vspace{-4mm}
%     \label{gyrocali}
% \end{figure}
\vspace{-1mm}
\subsection{Lower Calibration Frequencies for Higher Calibration Qualities} 
\vspace{-1mm}\label{boost_ori_2}
Accelerometer and magnetometer calibrations serve as drift suppressors for gyroscope integration.
% If the integration drives too far away from the right course, calibrations bring it back.
However, an assumption here is that calibrators should be more accurate than the integration.
% so that calibrations can improve the overall estimation.
If the integration is more accurate, while we let worse calibrators supervise the integration, calibrations would decrease orientation accuracy.
To demonstrate this speculation, we compare the error of gyro integration with the errors of gravity calibration and magnetic calibration, aggregated on 70 one-minute-long data traces.
\vspace{-1mm}
% The calibration-only method is only using accelerometer and magnetometer to come up with orientation estimation, which is just the same as performing complementary filter initialization on every timestep.

\begin{figure*}[h]
    % \hfill
    \vspace{-2mm}
    \begin{minipage}[t]{0.45\linewidth}
        \centering
        % \hspace{-0.3cm}
        % \vspace{-0.2cm}
        \includegraphics[width=1\linewidth]{fig/mobi_gyro_cali.pdf}
        \vspace{-4mm}
       \caption{Angular errors of gyroscope integration, accelerometer, and magnetometer.}
        % \vspace{-4mm}
        \label{gyrocali}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.47\linewidth}
        \centering
        % \hspace{-0.3cm}
        % \vspace{-0.2cm}
        \includegraphics[width=1\linewidth]{fig/sensys_kk.pdf}
        \vspace{-4mm}
        \caption{Orientation error with different gyroscope integration frequency $K_g$ and calibration frequency $K_c$.}
        \label{kk}
    \end{minipage}
    \Description[bruh]{bruh bruh}
    % \hfill
    \vspace{-3mm}
\end{figure*}

% \begin{figure}
%     \centering
%     \hspace{-0.3cm}
%     \vspace{-0.2cm}
%     \includegraphics[width=0.85\linewidth]{fig/sensys_kk.pdf}
%     \vspace{-1mm}
%     \caption{Orientation error with different gyroscope integration frequency $K_g$ and calibration frequency $K_c$.}
%     \vspace{-5mm}
%     \label{kk}
% \end{figure}

% \input{Ktable.tex}

As shown in Figure \ref{gyrocali}, gyroscope integration error accumulates at a rate of approximately 0.2°/s. 
If the gyroscope integration error starts from 0°, it would take more than 20 seconds for the accumulation to surpass the two calibrators' error.
It means if we perform calibration in the first several seconds, then we will calibrate a high-quality gyroscope integration result with two low-quality calibrators, which would degrade the overall orientation accuracy.
% quality to the level of the two calibrators.
This implies that it may not be wise to perform calibration too frequently. 
% Accelerometer and magnetometer are long-term accurate and gyroscope integration is short term accurate.
However, we notice, with our system's sampling interval being 20ms, both our calibration and integration frequencies are 50Hz by default.
This motivates us to tune the calibration frequency for complementary filter.
Figure \ref{gyrocali} is only a simplified demonstration.
In reality, gyroscope integration may not start from 0° error, and calibrators also have quality fluctuations.
Therefore, we conduct real experiments to find best calibration frequency.
We also test the frequency of gyroscope integration along the experiment.
We set a $K_{c}$ to control the calibration frequency
% in complementary filter
, as well as a $K_{g}$ to examine the effect of gyroscope integration frequency.
If the time step index $i$ is divided by $K_{c}$, complementary filter performs calibrations.
When $i$ is divided by $K_{g}$, complementary filter performs gyroscope integration.
When $i$ is divided by both $K_{g}$ and $K_{c}$, complementary filter performs both.

% 22.03238669	20.85566703	20.07721121	18.60999014	16.56250514	15.43572568	14.5617657	14.85124545	14.41010533	14.42195929	14.50770357	14.50375446	14.65517116	15.11037327	16.52809827	17.50233547



Figure \ref{kk} shows the influence of two frequencies on the error of complementary filter.
Darker block means higher error.
% We reach the lowest error when $K_{c}=24$.
\aliasSystem reaches the lowest error when $K_{c}=24$.
Given that our smartwatch's sampling rate is 50Hz, the best frequency for calibration is 2.0833Hz.
% verifying the long term accuracy of accelerometer and magnetometer.
We also see that the error is the lowest when $K_{g}$ is 1, meaning for gyroscope integration, high frequency is preferred. 
% verifying the short term accuracy of gyroscope integration.
Intuitively explaining, when we decrease the frequency of using magnetometer and accelerometer for calibration, we are decreasing the impact of the high-frequency noise in them (noisy even after basic anti-noising, due to constant variation in arm motion).
On the other hand, gyroscope is relatively less noisy thus fits high frequency usage.
When $K_{c} > 24$, the time resolution is too low to track the continuous changing of orientation.
% Finally, 
We adopt this modification for the complementary filter in \aliasSystem and set $K_{c}=24$, $K_{g}=1$. 
This experiment provides us an insight that it may be better to set $K_{c}>1$.
However, $K_{c}$ and $K_{g}$ could be related to the sensor noise level, thus if the system is to transform to other platform equipped with different IMU sensors, the best setting of $K_{c}$ and $K_{g}$ may need to be re-determined.
\vspace{-1mm}

% We name this modified complementary filter as NCF.
% Although $K_{c}=24$ and $K_{g}=3$ gives the lowest error, we still stick to $K_{g}=1$, because the difference is negligible, and we do want to maintain the output density of our system.
% With this design splitting $K_{c}=24$ and 
% This modification can easily be applied on complementary filter.
% with DB.

% 【CONFLICT】【CONFLICT】【CONFLICT】【CONFLICT】【CONFLICT】【CONFLICT】【CONFLICT】【CONFLICT】【CONFLICT】【CONFLICT】【CONFLICT】【CONFLICT】【CONFLICT】【CONFLICT】【CONFLICT】【CONFLICT】【CONFLICT】【CONFLICT】【CONFLICT】【CONFLICT】【CONFLICT】【CONFLICT】【CONFLICT】【CONFLICT】
% This Section~\ref{boost_ori_2} pursues higher calibration quality, while previous Section~\ref{boost_ori_1} sacrifice a little calibration quality for more opportunities, which seems inconsistent.
% However, this Section~\ref{boost_ori_2} focus on higher quality in short term (half a second, given $K_{c}=24$), while previous Section~\ref{boost_ori_1} increases the overall calibration opportunities at the cost of a little quality, for the entire time scope (10 $\sim$ 20 minutes).
% Therefore, they have no potential technical conflict. 










		


    % \hline
        %  Upgrades & pro version & without pro  \\
        % %  \\ \hline
        % database assisted & complementary filter+particle filter+DB pro: 22.6547° & complementary filter+particle filter+DB: 27.5631°\\ 
        % % \\ \hline
        % DB disabled & complementary filter+particle filter pro: 26.8866° & complementary filter+particle filter: 32.4920°\\
    %     \\
    % \hline

% \begin{table}
%     \begin{tabular}%{Performance gain of pro modification and DB}
%     Upgrades    & pro version             & without pro         &  &  \\
%     DB assisted & complementary filter+particle filter+DB pro: 22.6547° & complementary filter+particle filter+DB: 27.5631° &  &  \\
%     DB disabled & complementary filter+particle filter pro: 26.8866°     & complementary filter+particle filter: 32.4920°     &  &  \\
%                 &                         &                     &  & 
%     \end{tabular}
% \end{table}

% \subsubsection{Final Version: \aliasSystem}
% Based on \aliasSystem and putting everything together, we finish the design of \aliasSystem, which refines the database usage by improving the orientation and location inputs.
% We then conduct real experiments with extensive data, to examine the capability of \aliasSystem.



==> Solve.tex <==
% \section{Solution for Magnetic Calibration}





==> motivation.tex <==
% \section{Motivation}
% Inertial sensors enable orientation tracking without external infrastructures. Magnetometer plays an important roll among the three sensors. It provides an anchor direction to the geological North and thus provides
% People usually believe magnetometer points to North. However, magnetometer only measures the local magnetic field.
% Existing orientation inference algorithms that use magnetometers apply a strong assumption that the local magnetic field follows the same direction, to the geo-North.
% However, that assumption is not always true. 
% In many indoor scenarios geo-magnetic field is distorted by buildings. Metallic building structures may twist geo-magnetic field and change the strength and direction distribution of the magnet on different location. 
% % 画3-d磁场图，confer vs hw + hw2 + hw3

% Classic orientation inference algorithms may work outdoor, where the geo-magnetic field is free from distortion by buildings or metalic artifacts, but will fail terribly when the indoor magnet is distorted.
% % 给出经典算法在hw的实验结果说明一般算法受不了磁力高度扭曲的情况

% Unfortunately, most application that requires orientation works indoor, which calls on researchers to enable 
% 谷歌星空，VR控制，智能家居

==> observation.tex <==
% \section{Disclosing Magnetic Distortion}
% Magnetic field is the magnetic distribution across the space.
% The magnet distribution is related to location, while its temporal correlation is weak and can be ignored.
% To prove the weak temporal correlation of magnetic field.
% % 给实验结果证明distortion与时间无关
% Several researches also support that the magnetic field is almost eternal.
% % 引文章证明distortion与时间无关
% To 
